Chiral phase memory of twisted light through multiple scattering

Chiroptical signals, optical responses sensitive to molecular handedness, are rapidly suppressed by multiple scattering, fundamentally limiting their use in turbid media. Here we show that coupling molecular chirality to the topological structure of twisted light generates a protected phase observable that survives strong scattering. When Laguerre-Gaussian beams carrying orbital angular momentum propagate through chiral media, spin-orbit interaction converts circular birefringence into an azimuthal rotation of the helical wavefront. Remarkably, this chiral phase memory persists at scattering strengths that fully depolarize conventional beams, with the rotation magnitude preserved quantitatively between transparent solutions and strongly scattering tissue. The sign of the azimuthal rotation encodes molecular handedness: opposite enantiomers produce mirror-symmetric phase maps even after multiple scattering. Differential measurements between conjugate topological charges isolate the chiral contribution while cancelling achiral background, enabling the resolution of refractive-index changes of order 10-6. These results establish topological phase observables as robust carriers of weak chiral light-matter interactions in complex media, opening new routes for chiroptical spectroscopy and sensing beyond the ballistic-photon regime.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

